Sequence Diagram Test Case Specification and Virtual Integration Analysis using Timed-Arc Petri Nets

In this paper, we formally define Test Case Sequence Diagrams (TCSD) as an easy-to-use means to specify test cases for components including timing constraints. These test cases are modeled using the UML2 syntax and can be specified by standard UML-modeling-tools. In a component-based design an early identification of errors can be achieved by a virtual integration of components before the actual system is build. We define such a procedure which integrates the individual test cases of the components according to the interconnections of a given architecture and checks if all specified communication sequences are consistent. Therefore, we formally define the transformation of TCSD into timed-arc Petri nets and a process for the combination of these nets. The applicability of our approach is demonstrated on an avionic use case from the ARP4761 standard.

==> eptcsdata.tex <==
\providecommand{\firstpage}{17}
\providecommand{\publicationstatus}{B. Buhnova, L. Happe, J. Kofro\v{n}: \\
Formal Engineering Approaches to Software Components \\
and Architectures 2013 (FESCA'13)\\
EPTCS 108, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.108.2}{10.4204/EPTCS.108.2}}
\pdfoutput=1

